A Fast Algorithm for the Real-Valued Combinatorial Pure Exploration of Multi-Armed Bandit

We study the real-valued combinatorial pure exploration problem in the stochastic multi-armed bandit (R-CPE-MAB). We study the case where the size of the action set is polynomial with respect to the number of arms. In such a case, the R-CPE-MAB can be seen as a special case of the so-called transductive linear bandits. We introduce an algorithm named the combinatorial gap-based exploration (CombGapE) algorithm, whose sample complexity upper bound matches the lower bound up to a problem-dependent constant factor. We numerically show that the CombGapE algorithm outperforms existing methods significantly in both synthetic and real-world datasets.

==> _header.tex <==

\RequirePackage{fancyhdr}
% \fancypagestyle{plain}{%
% \fancyhf{}
% \lhead{\phone \\ % PHONE
% 	    \href{mailto:\email}{\email}} % EMAIL}
% 	\chead{%
% 	    \centering {\Large \bold\name} \\%
% 	    {\color{highlight} \large{\role}}}%
% 	    \rhead{
% 	    Portfolio: \href{https://mathtodata.com}{ MathtoData.com}\\ % Portfolio
% 	    \href{https://github.com/\github}{github.com/\github} \\% Github
% 	    \href{https://www.linkedin.com/in/\LinkedIn}{linkedin.com/in/\LinkedIn}} % LinkedIn
% \renewcommand{\headrulewidth}{2pt}% 2pt header rule
% \renewcommand{\headrule}{\hbox to\headwidth{%
%   \color{highlight}\leaders\hrule height \headrulewidth\hfill}}
% }
\pagestyle{plain}

\setlength{\headheight}{90pt}
\setlength{\headsep}{0pt}

\makeatletter
\let\ps@empty\ps@plain
\let\ps@firstpage\ps@plain
\makeatother

==> sections/closing.tex <==
% The next paragraph should focus on another key achievement or skill that is relevant to the position. Instead of repeating details from your resume, expand on specific stories or anecdotes that display your fitness for the role. Again, focus on stories that demonstrate the skills and qualifications outlined in the job description.

% If you’re changing careers, this is a good opportunity to talk about transferable skills or relatable experiences from your career.

% https://www.indeed.com/career-advice/resumes-cover-letters/how-to-write-a-cover-letter


% Achieving ambitious marketing goals is always a top priority, and I am always looking out for the best interests of the company. I enjoy delivering marketing presentations to potential clients and focusing on the strengths of an organization. My marketing skills at River Tech enabled the company to experience new levels of success and a 45\% increase in customer engagement. I am never satisfied with the status quo, and I believe that a company should continually look for ways to improve and reach new clients through innovative campaigns.

==> sections/opening.tex <==
% In the first paragraph of your letter, mention the job title for which you’re applying and where you saw the position posting. Explain your specific interest in the role and company so the reader knows you’ve done your research and have genuine interest. Briefly state the main experience or qualification you have that makes you a good fit. The first section of your cover letter is also the first impression the reader will have of you, so it is important to appeal to that person quickly and succinctly. 

% https://www.indeed.com/career-advice/resumes-cover-letters/how-to-write-a-cover-letter 



% I'm excited to apply for the \position\;position at \company\;that I found \source. 
% \companynews\,I believe my skills in video and animation provide a significant advantage for creating a successful launch. As a longtime fan of your products, I'm thrilled at the opportunity to bring my unique style and passion for beachwear to the company.
Please find our manuscript entitled 
\begin{center}
    A Fast Algorithm for the Real-Valued Combinatorial Pure Exploration of Multi-Armed Bandit
\end{center}
by Shintaro Nakamura and Masashi Sugiyama. We indicate our response to the review comments and the changes we have made in the revised manuscript. \par
Thanks to reviewer 1, we have found a mistake in our theoretical analysis and found out that the CombGapE algorithm is not optimal, which means that it does not match the lower bound shown in (8). We revised our theoretical analysis and showed that the CombGapE algorithm matches the lower bound up to a problem-dependent constant factor. This upper bound is the same as that of the TSExplore algorithm. Also, as mentioned in the first comment of Reviewer 1, it is an interesting future work to construct an optimal algorithm that does not enumerate all the feasible actions in the action set. Another possible direction is to derive a lower bound which assumes that the player cannot enumerate all the feasible actions in the action set.  \par
Second, we have conducted an additional experiment based on real-world data. In the experiment section, we showed that the CombGapE algorithm can find the best transportation matrix of the optimal transport problem and that it outperforms existing methods significantly. Related to the second question of Reviewer 2, one may refer to the paper \emph{Fixed-Budget Real-Valued Combinatorial Pure Exploration of Multi-Armed Bandit} by Shintaro Nakamura and Masashi Sugiyama, which studies the fixed-budget setting of R-CPE-MAB.  \par


==> sections/second.tex <==
% Your second paragraph should be a brief overview of your background as is relevant to the position. Here, you should include key achievements, skills and specialties that make you particularly suited to perform well in the position. Focus on one or two and provide specific details about your success including measurable impacts you made.

% Pay close attention to keywords listed in the job description and include those that you identify with in the body of your cover letter. You should only include information about your most recent one or two professional experiences.

% https://www.indeed.com/career-advice/resumes-cover-letters/how-to-write-a-cover-letter

% As the Director of Human Resources at Wes Morgan Philips, I was a key senior leader in the organization and was responsible for improving the efficiency and performance of the company's 540 employees. Before that, I worked in human resources, equal employment opportunity and diversity for Jenkins Technology Solutions, Inc. At Jenkins Technology Solutions Inc., I developed an employee retention plan that involved the creation of a wellness program, an internal training program and a promotions selection process, which led to a 50\% reduction in the overall employee turnover rate.


==> sections/signoff.tex <==
% You should end your cover letter with a paragraph that summarizes the reasons you are applying for the role and why you would be a great fit. Keep the cover letter conclusion brief and explain that you look forward to hearing from the employer with the next steps. End with your signature at the bottom.

% https://www.indeed.com/career-advice/resumes-cover-letters/how-to-write-a-cover-letter



% Thank you for your time and consideration. I'm looking forward to learning more details about the \position\;position at \company. Growth is essential to my continued success, and I'm excited for the chance to be a part of \company's industry-leading team. My proven track record and \company's quality products are a winning combination for increasing the company's market share.


